Beyond the Delay-Doppler Domain: A Time-Frequency Framework for Low-Overhead, Scalable OTFS Channel Estimation

Most works on pilot-aided orthogonal time frequency space (OTFS) channel estimation operate in the delay-Doppler (DD) domain, where embedded-pilot guard regions must cover the unknown maximum delay-Doppler spread, causing high overhead that worsens with antenna scaling: per-antenna guard regions increase overhead with the number of transmit antennas, while shared guard regions avoid this but introduce pilot contamination. Fractional Doppler further reduces DD-domain sparsity and increases estimation complexity. This paper shows that the time-frequency (TF) representation provides a low-overhead, scalable framework for OTFS channel estimation based on physical scatterer parameters (angle, delay, Doppler, and gain). We derive exact TF- and DD-domain input-output relationships under fractional Doppler. The TF expression decomposes the received signal into a desired component, identical in form for integer and fractional Doppler, and an explicitly characterized interference term; this Doppler-invariant structure enables scalable TF-domain estimation. This motivates a TF-domain pilot design using private TF bins protected by TF/DD guard bins, preserving cross-antenna pilot orthogonality with overhead that depends only on the number of pilots, not the array size. We then develop a low-complexity coarse-to-fine estimation method combining discrete Fourier transform (DFT)-based coarse estimation with dimensionality-reduced sparse recovery. The exact DD-domain expression provides the signal model for data-symbol recovery and explains why DD-domain estimation complexity grows substantially under fractional Doppler. Simulations show accurate channel state information (CSI) estimation under integer and fractional Doppler, robustness to pilot pollution, and scalability to large arrays with substantially lower overhead and complexity than existing schemes.

==> Format.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Packages to Load
%% Text and Math Environment Packages
\RequirePackage{csquotes} %Package to Facilities Quotations
% \RequirePackage[backend=biber, style=ieee, sorting=ynt]{biblatex}
\RequirePackage[noadjust]{cite}
% \RequirePackage[english]{babel} %Multilingual Support Must Load the First
% \RequirePackage[utf8]{inputenc} %utf8 Support. Preloaded in Distribution
\RequirePackage[T1]{fontenc} %Better Font Encoding for T1 Type Font
\RequirePackage[shortlabels, inline]{enumitem} %Conflict with Beamer
\RequirePackage[table, svgnames]{xcolor} %Beamer Has This by Default
\RequirePackage[most]{tcolorbox} %Customized Box. Must Load after xcolor
\RequirePackage{mathtools} %Customize Math Symbols and Theorems
\RequirePackage{amsthm, thmtools, thm-restate} %Better Theorems
% \RiquirePackage{amsmath} %Loaded by mathtools
\RequirePackage{amssymb} %Conflict with Fonts
% \RequirePackage{Fonts} %Must Load after tcolorbox and amsthm
% \let\openbox\undefined %Fix Some Font Issues
\RequirePackage{mleftright} %Fixes Some Math Spacing Issues
\RequirePackage{siunitx}
\RequirePackage{bm} %Boldface Math, Load after Other Math Font Packages
\RequirePackage{microtype} %Better Font Spacing
\RequirePackage{fontawesome5} % 

%% Table Packages
\RequirePackage{tabularx} %Including Tabular with More Space Option
% \RequirePackage{colortbl} %Package to Use Color in Tables. Replaced by table option of xcolor
\RequirePackage{multirow} %Package to Use Multirow in Tables
\RequirePackage{multicol} %Package to Use Multicols
\RequirePackage{array} %Math and More Spacing Support in Tables

%% Graphics Packages
\RequirePackage{epstopdf} %Package to Convert eps to pdf in pdfLatex
\RequirePackage{transparent} %Transparent Images
\RequirePackage{graphicx} %Graphics Backend with key-value Arguments
\RequirePackage[export]{adjustbox} %More Arguments for includegraphics
\RequirePackage[caption=false, font=footnotesize]{subfig}

% %% IEEE Figure Style
% \makeatletter
% \let\MYcaption\@makecaption
% \makeatother

% \RequirePackage[font=footnotesize]{subcaption}

% \makeatletter
% \let\@makecaption\MYcaption
% \makeatother

%% Code Packages
% \RequirePackage{listings} %Loaded by tcolorbox and also no need of minted.
\RequirePackage{algorithm} %Package to Insert Algorithm
\RequirePackage{algpseudocode} %Package to Insert Algorithm

%% Other Packages
\RequirePackage{xspace} %Package to Add Space after Macros
% \RequirePackage{calc} %Package of Calculation in Latex
% \RequirePackage{rotating} %Package to Rotate Objects
% \RequirePackage{pgf, tikz} %Package to Draw Figures.
% \RequirePackage{keyval}
\RequirePackage{hyperref} %Beamer Has This by Default.
\RequirePackage{bookmark}
\RequirePackage{orcidlink}
\RequirePackage[capitalise,nameinlink]{cleveref} %Must Load after others. Conflict with Beamer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
